Large Structures and Galaxy Evolution in COSMOS at z < 1.1

We present the first identification of large-scale structures (LSS) at z $< 1.1$ in the Cosmic Evolution Survey (COSMOS). The structures are identified from adaptive smoothing of galaxy counts in the pseudo-3d space ($\alpha,\delta$,z) using the COSMOS photometric redshift catalog. The technique is tested on a simulation including galaxies distributed in model clusters and a field galaxy population -- recovering structures on all scales from 1 to 20\arcmin without {\it a priori} assumptions for the structure size or density profile. Our procedure makes {\bf no} {\it a priori} selection on galaxy spectral energy distribution (SED, for example the Red Sequence), enabling an unbiased investigation of environmental effects on galaxy evolution. The COSMOS photometric redshift catalog yields a sample of $1.5\times10^5$ galaxies with redshift accuracy, $\Delta z_{FWHM}/(1+z) \leq 0.1$ at z $< 1.1$ down to I$_{AB} \leq 25$ mag. Using this sample of galaxies, we identify 42 large-scale structures and clusters. abstract truncated for astroph 25 line limit -- see preprint

==> title_authors <==
Large Structures and Galaxy Evolution in COSMOS at z < 1.1
 

N. Scoville,H. Aussel,A. Benson,A. Blain,D. Calzetti,P. Capak,R. S. Ellis,A. El-Zant,A. Finoguenov,M. Giavalisco,L. Guzzo,G. Hasinger,J. Koda,O. Lefevre,R. Massey,H. J. McCracken,B. Mobasher,A. Renzini,J. Rhodes,M. Salvato,D. B. Sanders,S. S. Sasaki,E. Schinnerer,K. Sheth,P. L. Shopbell,Y. Taniguchi,J. E. Taylor,D. J. Thompson


 We present the first identification of large-scale structures (LSS) at z $< 1.1$ in the Cosmic Evolution Survey (COSMOS).
 The structures are identified from adaptive smoothing of galaxy counts in 
 the pseudo-3d space ($\alpha,\delta$,z) using the COSMOS photometric redshift catalog.
 The technique is tested on a simulation including galaxies distributed
 in model clusters and a field galaxy population -- recovering structures on all scales from 1 
 to 20\arcmin~without {\it a priori} assumptions for the structure size or density profile. 
 Our procedure makes {\bf no} {\it a priori} selection on galaxy spectral energy distribution (SED,
 for example the Red Sequence), enabling an unbiased investigation of environmental 
 effects on galaxy evolution. 
 
 The COSMOS photometric redshift catalog yields a sample of $1.5\times10^5$ galaxies with  
 redshift accuracy, $\Delta z_{FWHM}/(1+z) \leq 0.1$ at z $< 1.1$ down to  I$_{AB} \leq 25$ mag. 
 Using this sample of galaxies, we identify  42 large-scale structures and clusters. 
 Projected surface-density maps for the structures indicate multiple 
 peaks and internal structure in many of the most massive LSS. 
 The stellar masses (determined from the galactic SEDs) for the LSS range 
 from M$_* \sim 10^{11}$  up to $\sim3\times10^{13}$ \msun. Five LSS have 
total stellar masses exceeding $10^{13}$ \msun. (Total masses including non-stellar 
baryons and dark matter are expected to be $\sim 50 \rightarrow 100$ times greater.) 
The derived mass function for the LSS is consistent (within the expected Poisson and cosmic variances) 
with those derived from optical and X-ray studies at lower redshift.  

To characterize structure evolution and for comparison 
with simulations, we compute a new statistic -- the area filling factor  as a function of the overdensity value compared to the 
mean at surface overdensity ($f_A(\Sigma/{\overline{\Sigma}(z)}$).  The observationally determined f$_A$ 
has less than 1\% of the surface area (in each redshift slice) with overdensities exceeding 10:1
and  evolution to 
higher overdensities is seen at later epochs (lower z) -- both characteristics are in  good agreement 
with what we find using similar processing on the Millennium Simulation. Although similar variations in the filling factors 
as a function of overdensity and redshift 
are seen in the observations and simulations, we do find that the observed distributions reach 
higher overdensity than the simulation, perhaps indicating  
over-merging in the simulation. 

 All of the LSS
 show a dramatic preference for earlier spectral energy distribution (SED type) galaxies in the denser regions of  the 
 structures, independent of redshift. The SED types in the central 1 Mpc and 1 -- 5 Mpc regions of each structure
 average about 1 SED type earlier than the mean type at the same 
 redshift, corresponding to a stellar population age difference of $\sim$2 -- 4 
 billion years at z = 0.3 to 1. 
   
We also investigate the evolution of key galactic properties -- mass, luminosity, SED 
and star formation rate (SFR) -- with redshift and environmental density as derived from  
 overdensities in the full pseudo 3-d cube. Both the maturity of the stellar populations and the 'downsizing' 
of SF in galaxies vary strongly with redshift (epoch) and environment. For a very broad mass range (10$^{10} -- 10^{12}$\msun), we find that galaxies in dense 
environments tend to be older -- this is not just restricted to the most massive galaxies. And in low density environments, 
the most massive galaxies appear to have also been formed very early (z $> 2$), compared 
to the lower mass galaxies there.
Over the range z $< 1.1$, we do not see evolution in the 
mass of galaxies by more than a factor $\sim 2$ separating  active and inactive star-forming galaxy populations. 

